Learning to Generate Task-Specific Adapters from Task Description

Pre-trained text-to-text transformers such as BART have achieved impressive performance across a range of NLP tasks. Recent study further shows that they can learn to generalize to novel tasks, by including task descriptions as part of the source sequence and training the model with (source, target) examples. At test time, these fine-tuned models can make inferences on new tasks using the new task descriptions as part of the input. However, this approach has potential limitations, as the model learns to solve individual (source, target) examples (i.e., at the instance level), instead of learning to solve tasks by taking all examples within a task as a whole (i.e., at the task level). To this end, we introduce Hypter, a framework that improves text-to-text transformer's generalization ability to unseen tasks by training a hypernetwork to generate task-specific, light-weight adapters from task descriptions. Experiments on ZEST dataset and a synthetic SQuAD dataset demonstrate that Hypter improves upon fine-tuning baselines. Notably, when using BART-Large as the main network, Hypter brings 11.3% comparative improvement on ZEST dataset.

==> figures_input/adapter.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.3\textwidth]{figures/ZS-transformer-layer.pdf}
    \vspace{-0.1cm}
    \caption{\textbf{Simplified Adapters Used in This Work.} An adapter includes two linear layers, $(\mathbf{W}_{id}, \mathbf{b}_{id})$ and $(\mathbf{W}_{iu}, \mathbf{b}_{iu})$, separated by a non-linear activation. An adapter can be plugged into a transformer layer, by adding it after the first feed-forward layer. Figure adapted from \cite{pmlr-v97-houlsby19a}.}
    \vspace{-0.4cm}
    \label{fig:adapter}
\end{figure}

==> figures_input/arch.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/ZS.pdf}
    % \vspace{-0.4cm}
    \caption{\textbf{Overview of \textsc{Hypter} Framework.} The hypernetwork generates adapters from task descriptions, and insert them to transformer layers in the main network. The main network is ready to inference on the described task.}
    \label{fig:arch}
    \vspace{-0.5cm}
\end{figure}

==> tables/input_output_format.tex <==
\begin{table}[t]
    \centering
    \scalebox{0.65}{
    \begin{tabular}{p{10cm}}
    \toprule
        \makecell[l{p{10cm}}]{
        ZEST\\
        \textbf{Input:} zest question: What accessibility services does this national park offer? zest context: Mammoth Cave National Park is pleased to offer sign interpreter services for cave and surface activities to visitors free of charge.  Arrangements can be made by contacting the park at the number located below. ...\\
        \textbf{Output:} sign interpreter services for cave and surface activities}  \\
    \midrule
         \makecell[l{p{10cm}}]{
         ZSRE (without description)\\
        \textbf{Input:} Waldo Maguire [SEP] employer \\
        \textbf{Output:} BBC}  \\
    \midrule
         \makecell[l{p{10cm}}]{
         ZSRE (with description)\\
        \textbf{Input:} Waldo Maguire [SEP] employer [SEP] person or company that employs workers\\
        \textbf{Output:} BBC}  \\
    \bottomrule
    \end{tabular}
    }
    % \vspace{-0.2cm}
    \caption{\textbf{Examples of the input and targets.} Task descriptions are included as part of the input as ``prompt''. \xiang{can move to appendix, and enrich Fig. 1}}\label{tab:schematic}
\end{table}

==> tables/zest.tex <==
\begin{table}[t]
\centering
\vspace{-0.0cm}
\scalebox{0.59}{
\begin{tabular}{lcccccccccccc}
\toprule
                       & \multicolumn{3}{c}{ZEST-Dev} & \multicolumn{3}{c}{ZEST-Test}  \\
Model                   & Mean-F1 & C@75   & C@90  & Mean-F1 & C@75   & C@90  \\
\midrule
Bart-Base & 29.72  & 7.87  & \textbf{4.05}  & 31.97 & \textbf{7.03}  & 2.23  \\
\ \ + \textsc{Hypter}    & \textbf{29.81}  &  \textbf{8.67} & \textbf{4.05} & \textbf{32.32} &  6.72 & \textbf{2.53} \\
\midrule
Bart-Large (reported)  & 40     & 13     & 8     & 37.93  & 11.19  & 3.96 \\
Bart-Large & 42.10  & 16.72  & 8.85  & 40.13  & 10.91 & 3.98  \\
\ \ + \textsc{Hypter}    & \textbf{43.50}  & \textbf{17.46} & \textbf{9.64} & \textbf{40.41}  & \textbf{11.35} & \textbf{4.43}  \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Performance on ZEST dataset.} ``C@75/90'' refers to Competence@75/90 metric.}\label{tab:zest}
\end{table}

==> tables/zsre.tex <==
\begin{table}[t]
\centering
\scalebox{0.6}{
\begin{tabular}{lcc}
\toprule
                       & \multicolumn{1}{c}{ZSRE-Dev} & \multicolumn{1}{c}{ZSRE-Test} \\
\midrule
\textit{Without Description.} \\
Bart-Base  & 1.83 & 9.10 \\
\ \ + \textsc{Hypter}    & 1.96 & 9.16 \\
Bart-Large (reported)  & 3.03 & 9.14 \\
Bart-Large  & 2.95 & 9.93 \\
\ \ + \textsc{Hypter}  & 2.98 & 9.95 \\
\midrule
\textit{With Description.} \\
Bart-Base & 2.34 & 9.57 \\
\ \ + \textsc{Hypter}    & 2.60 & 9.81 \\
Bart-Large  & 3.33 & 11.44    \\
\ \ + \textsc{Hypter}  & \textbf{3.57} & \textbf{11.48}  \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Performance on ZSRE dataset.} ``Bart-Large (reported)'' results are from \cite{petroni2020kilt}.}\label{tab:zsre}
\end{table}
